SemVecNet: Generalizable Vector Map Generation for Arbitrary Sensor Configurations

Vector maps are essential in autonomous driving for tasks like localization and planning, yet their creation and maintenance are notably costly. While recent advances in online vector map generation for autonomous vehicles are promising, current models lack adaptability to different sensor configurations. They tend to overfit to specific sensor poses, leading to decreased performance and higher retraining costs. This limitation hampers their practical use in real-world applications. In response to this challenge, we propose a modular pipeline for vector map generation with improved generalization to sensor configurations. The pipeline leverages probabilistic semantic mapping to generate a bird's-eye-view (BEV) semantic map as an intermediate representation. This intermediate representation is then converted to a vector map using the MapTRv2 decoder. By adopting a BEV semantic map robust to different sensor configurations, our proposed approach significantly improves the generalization performance. We evaluate the model on datasets with sensor configurations not used during training. Our evaluation sets includes larger public datasets, and smaller scale private data collected on our platform. Our model generalizes significantly better than the state-of-the-art methods.

==> backup.tex <==
% We introduce a vector map generation approach using a BEV semantic map, diverging from neural network methods. 
% Diverging from approaches using neural networks to transform features into BEV, our approach combines LiDAR data and sensor intrinsics and extrinsics to create a consistent, sensor-agnostic BEV representation. This method, focusing on 3D geometry, mitigates overfitting and adapts to varying sensor setups, ensuring robust generalization. By standardizing input through this ego-centric BEV map, our model demonstrates enhanced adaptability in diverse real-world scenarios, particularly in vector map generation with unseen sensor platforms.

% We deviate from the conventional image view encoder-feature space-vector map decoder architecture by using a semantic map instead of a learned intermediate representation. This allows for cross-dataset generalization by having a geometrically standardized intermediate representation.

% GPT: In this paper, we present a novel approach for generating vector maps by incorporating an intermediate Bird's Eye View (BEV) semantic representation, which ensures robust generalization across diverse sensor configurations. Our methodology diverges from conventional neural network-based image projections, instead utilizing a combination of LiDAR data, camera transformation matrices, and sensor extrinsics to construct an ego-centric BEV semantic map. This map, being a 2D projection of semantic world features, exhibits minimal variation despite changes in sensor setups, thus making it configuration agnostic. By shifting the computational complexity to the Semantic Mapping pipeline, which is inherently 3D-geometry based, we effectively reduce the overfitting risks associated with learned feature spaces in typical encoder-to-feature space-to-decoder architectures. The semantic map's consistent quality across varying sensor extrinsics and intrinsics, combined with a 360-degree Field of View (FOV) for cameras, provides a standardized input to the neural network. This enhances adaptability and applicability of our model in diverse real-world scenarios, especially in the task of vector map generation, where generalizability to unseen sensor platforms is crucial.

% Naru: Rather than directly projecting images into a Bird's Eye View (BEV) feature space using neural networks, our approach capitalizes on LiDAR data and sensor extrinsics to construct an ego-centric BEV semantic map. This semantic map exhibit minimal variation across various sensor configurations and serves as the input to our neural network. 

% By adopting this strategy, we strategically shift the burden of handling changes in extrinsics and intrinsics onto the Semantic Mapping pipeline, rather than burdening the Neural Network directly. 

% The Semantic Mapping pipeline, being entirely 3D-geometry based, ensures robust generalization to unseen sensor configurations. This is facilitated by maintaining a $360\degree$ Field of View (FOV) for the cameras and utilizing dense LiDAR data. The resulting semantic maps exhibit minimal variation across various sensor configurations, providing a standardized input to the neural network and enhancing the model's adaptability to diverse real-world scenarios.

% Shanky: Rather than using neural networks to project images into a learned feature space, we utilize camera transformation matrices and LiDAR data to project images into a BEV semantic map. Learned feature spaces overfit to the sensor configuration during training, while the BEV semantic map is constant and configuration agnostic as it is a BEV 2D projection of semantic world features.


% Many approaches follow an encoder to feature space to decoder architecture, where the encoder takes images to a BEV feature space, and the decoder takes this feature space 

% Henry: We leverage an intermediate BEV semantic representation that takes different sensor configurations into account to tackle the problem of vector map generation. Compared to approaches using neural networks to generate BEV features, our approach is more generalizable.


% Utilizing this semantic map as input allows the network to generalize to unseen sensor configurations as the burden of dealing with the change in extrinsics is shifted to the Semantic Mapping pipeline. As such it does not fit to the extrinsic parameters of the training set

% based on any specific intrinsic and extrinsic parameters, allowing it to generalize to other sensor configuration.

% leverages a semantic map as an intermediate representation that is not dependant on learning from a specific extrinsic configuration.



% These include the utilization of coordinate transformation matrices provided by the autonomous driving platform for direct projection, the usage of the semantic segmentation backbone's confusion matrix for probabilistic noise correction, and the incorporation of a Bird's Eye View (BEV) semantic map as an intermediate representation. These strategies enhance our model's ability to generalize to unseen sensor configurations.


% \item \textbf{Qualitative Result for Real-World Data: } In addition to testing on recognized datasets, we also generate results from data we collected from UC San Diego campus, further showing the transferable performance of our pipeline even without available training data.


% However, existing works suffer from the inability to generalize across different sensor setups as they tend to overfit to the extrinsics of the sensor configuration and also the transformation from image frame to map coordinate frame instead of utilizing the coordinate transformation between sensor and the world. 

% Current methodologies face a notable challenge in achieving generalization across diverse sensor setups. This limitation arises from a tendency to overfit to specific sensor extrinsics and focus predominantly on the transformation from the image frame to the map coordinate frame, neglecting the broader and crucial aspect of incorporating the comprehensive coordinate transformation between the sensor and the world. As a consequence, these models struggle to adapt effectively to varying sensor configurations, compromising their ability to perform reliably in diverse real-world scenarios."

% To address the generalization issue in vector map creation approaches, we propose to combine semantic mapping that consider intrinsic and extrinsic variation to generate an intermediate semantic map, then decode the semantic map into the vector representations. 
